Scheduled Intrinsic Drive: A Hierarchical Take on Intrinsically Motivated Exploration

Exploration in sparse reward reinforcement learning remains an open challenge. Many state-of-the-art methods use intrinsic motivation to complement the sparse extrinsic reward signal, giving the agent more opportunities to receive feedback during exploration. Commonly these signals are added as bonus rewards, which results in a mixture policy that neither conducts exploration nor task fulfillment resolutely. In this paper, we instead learn separate intrinsic and extrinsic task policies and schedule between these different drives to accelerate exploration and stabilize learning. Moreover, we introduce a new type of intrinsic reward denoted as successor feature control (SFC), which is general and not task-specific. It takes into account statistics over complete trajectories and thus differs from previous methods that only use local information to evaluate intrinsic motivation. We evaluate our proposed scheduled intrinsic drive (SID) agent using three different environments with pure visual inputs: VizDoom, DeepMind Lab and DeepMind Control Suite. The results show a substantially improved exploration efficiency with SFC and the hierarchical usage of the intrinsic drives. A video of our experimental results can be found at https://youtu.be/b0MbY3lUlEI.

==> apps/app-infrastructure.tex <==
%\section{Appendix: Computing Infrastructure}
%
%To generate our results we used two machines that run Ubuntu 16.04. 
%Each machine has 4 GeForce Titan X (Pascal) GPUs. On one machine we run 4 experiments in parallel, each experiment on a separate GPU.

==> apps/app-model.tex <==
\section{Appendix: Model Architecture}
\label{app:model}

We use the same model architecture as depicted in Fig. \ref{fig:model} across all $3$ sets of experiments.

\begin{figure}[t]
\center
    \includegraphics[width=0.7\columnwidth]{imgs/model}
    \caption{
        Model architecture for the \textbf{SID (M, SFC)} agent.
        Components with color yellow are randomly intialized and not trained during learning.
    }
    \label{fig:model}
\end{figure}

ReLU activation is added after every layer except for the last layers of each dashed blocks in the above figure.
For the experiments with the ICM \citep{pathakICMl17curiosity},
we added BatchNorm \citep{ioffe2015batch} before activation for the embedding of the ICM module following the original code released by the authors.
Code is implemented in pytorch \citep{paszke2017automatic}.



==> apps/app-rewardnorm.tex <==
\section{Appendix: Reward Normalization}
\label{app:rewardnorm}

Most network parameters are shared for estimating the expected  discounted return of the intrinsic and extrinsic rewards. The scale of the rewards has a big influence on the scale of the gradients for the network parameters. Hence, it is important that the rewards are roughly on the same scale, otherwise effectively different learning rates are applied.
The loss of the network comes from the regression on the Q-values, which approximate the expected return. So our normalization method aims to bring the discounted return of both tasks into the same range.
To do so we first normalize the intrinsic rewards by dividing them by a running estimate of their standard deviation.
We also keep a running estimate of the mean of this normalized reward and denote it $r_I'$.  Since every time step an intrinsic reward is received we estimate the discounted return via the geometric series.
We scale the extrinsic task reward that is always in $\{0,1\}$ with
$\eta \frac{r_I'}{1-\gamma_I}$, where $\gamma_I$ is the discount rate for the intrinsic reward. Furthermore, $\eta$ is a hyperparameter which takes into account that for Q-values from states more distant to the goal the reward is discounted with the discount rate for the extrinsic reward depending on how far away that state is. In our experiments we set $\eta = 3$ (Appendix \ref{app:training}).

